Online learning techniques for prediction of temporal tabular datasets with regime changes

The application of deep learning to non-stationary temporal datasets can lead to overfitted models that underperform under regime changes. In this work, we propose a modular machine learning pipeline for ranking predictions on temporal panel datasets which is robust under regime changes. The modularity of the pipeline allows the use of different models, including Gradient Boosting Decision Trees (GBDTs) and Neural Networks, with and without feature engineering. We evaluate our framework on financial data for stock portfolio prediction, and find that GBDT models with dropout display high performance, robustness and generalisability with reduced complexity and computational cost. We then demonstrate how online learning techniques, which require no retraining of models, can be used post-prediction to enhance the results. First, we show that dynamic feature projection improves robustness by reducing drawdown in regime changes. Second, we demonstrate that dynamical model ensembling based on selection of models with good recent performance leads to improved Sharpe and Calmar ratios of out-of-sample predictions. We also evaluate the robustness of our pipeline across different data splits and random seeds with good reproducibility.

==> temp.tex <==

%% Performance 
\begin{table}[htb!]
%\begin{tabular}{|l|l|l|l|l|l|}
(a) LightGBM-dart without FE 
\\
\begin{center}
\resizebox{.8\linewidth}{!}{
\begin{tabular}{|l|l|r|r|r||r|r|}
\hline
Regime                    & Feature Neutral & Mean & Volatility & Max Draw & Sharpe & Calmar \\ \hline
\multirow{2}{*}{All}      & Yes            & 0.0215                    & 0.0182                          & 0.1153                        & 1.1806                      & 0.1865                      \\ \cline{2-7} 
                          & No             & 0.0278                    & 0.0284                          & 0.1622                        & 0.9791                      & 0.1714                      \\ \hline
\multirow{2}{*}{High Vol} & Yes            & 0.0227                    & 0.0163                          & 0.0223                        & 1.3888                      & 1.0179                      \\ \cline{2-7} 
                          & No             & 0.0314                    & 0.0251                          & 0.0657                        & 1.2510                      & 0.4779                      \\ \hline
\multirow{2}{*}{Low Vol}  & Yes            & 0.0206                    & 0.0195                          & 0.1153                        & 1.0576                      & 0.1787                      \\ \cline{2-7} 
                          & No             & 0.0252                    & 0.0305                          & 0.1622                        & 0.8257                      & 0.1554                      \\ \hline
\end{tabular}
}
\end{center}
\bigskip
(b) LightGBM-gbdt without FE
\\
\begin{center}
\resizebox{.8\linewidth}{!}{
\begin{tabular}{|l|l|r|r|r||r|r|}
\hline
Regime                    & Feature Neutral & Mean & Volatility & Max Draw & Sharpe & Calmar \\ \hline
\multirow{2}{*}{All}      & Yes            & 0.0204                    & 0.0211                          & 0.1998                        & 0.9665                      & 0.1021                      \\ \cline{2-7} 
                          & No             & 0.0262                    & 0.0321                          & 0.2378                        & 0.8140                      & 0.1102                      \\ \hline
\multirow{2}{*}{High Vol} & Yes            & 0.0217                    & 0.0198                          & 0.0364                        & 1.0953                      & 0.5962                      \\ \cline{2-7} 
                          & No             & 0.0308                    & 0.0293                          & 0.1123                        & 1.0497                      & 0.2743                      \\ \hline
\multirow{2}{*}{Low Vol}  & Yes            & 0.0194                    & 0.0220                          & 0.1998                        & 0.8820                      & 0.0971                      \\ \cline{2-7} 
                          & No             & 0.0227                    & 0.0338                          & 0.2378                        & 0.6727                      & 0.0955                      \\ \hline
\end{tabular}
}
\end{center}

\bigskip
(c) MLP without FE
\\
\begin{center}
\resizebox{.8\linewidth}{!}{
\begin{tabular}{|l|l|r|r|r||r|r|}
\hline
Regime                    & Feature Neutral & Mean & Volatility & Max Draw & Sharpe & Calmar \\ \hline
\multirow{2}{*}{All}      & Yes            & 0.0179                    & 0.0203                          & 0.2606                        & 0.8798                      & 0.0687                      \\ \cline{2-7} 
                          & No             & 0.0258                    & 0.0289                          & 0.1668                        & 0.8931                      & 0.1547                      \\ \hline
\multirow{2}{*}{High Vol} & Yes            & 0.0196                    & 0.0193                          & 0.0326                        & 1.0191                      & 0.6012                      \\ \cline{2-7} 
                          & No             & 0.0298                    & 0.0276                          & 0.1247                        & 1.0802                      & 0.2390                      \\ \hline
\multirow{2}{*}{Low Vol}  & Yes            & 0.0165                    & 0.0210                          & 0.2606                        & 0.7875                      & 0.0633                      \\ \cline{2-7} 
                          & No             & 0.0228                    & 0.0296                          & 0.1668                        & 0.7721                      & 0.1367                      \\ \hline
\end{tabular}
}
\end{center}
\caption{\textbf{The effect of standard feature projection.} Performance of different ML methods on the Numerai dataset over the test period (2014-06-27 to 2022-09-23) with and without feature projection under different market regimes: the whole test period (All), high volatility regime (High Vol), and low volatility regime (Low Vol). } 
\label{table:numerai-v4-benchmark-test-FNC}
\end{table}







% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
Model                          & Average                           &      & Mean   & Volatility & Max Draw & Sharpe & Calmar \\ \hline
\multirow{4}{*}{LightGBM-dart} & \multirow{2}{*}{Over Models}      & Mean & 0.0255 & 0.0259     & 0.1500   & 0.9832 & 0.1704 \\ \cline{3-8} 
                               &                                   & S.D. & 0.0002 & 0.0001     & 0.0081   & 0.0094 & 0.0102 \\ \cline{2-8} 
                               & \multirow{2}{*}{Over Predictions} & Mean & 0.0276 & 0.0282     & 0.1605   & 0.9765 & 0.1721 \\ \cline{3-8} 
                               &                                   & S.D. & 0.0002 & 0.0001     & 0.0087   & 0.0089 & 0.0104 \\ \hline
\multirow{4}{*}{LightGBM-gbdt} & \multirow{2}{*}{Over Models}      & Mean & 0.0253 & 0.0308     & 0.2233   & 0.8196 & 0.1134 \\ \cline{3-8} 
                               &                                   & S.D. & 0.0001 & 0.0002     & 0.0080   & 0.0062 & 0.0044 \\ \cline{2-8} 
                               & \multirow{2}{*}{Over Predictions} & Mean & 0.0260 & 0.0319     & 0.2306   & 0.8161 & 0.1131 \\ \cline{3-8} 
                               &                                   & S.D. & 0.0001 & 0.0002     & 0.0083   & 0.0061 & 0.0044 \\ \hline
\multirow{4}{*}{MLP}           & \multirow{2}{*}{Over Models}      & Mean & 0.0231 & 0.0259     & 0.1490   & 0.8922 & 0.1550 \\ \cline{3-8} 
                               &                                   & S.D. & 0.0003 & 0.0003     & 0.0055   & 0.0095 & 0.0065 \\ \cline{2-8} 
                               & \multirow{2}{*}{Over Predictions} & Mean & 0.0254 & 0.0284     & 0.1610   & 0.8930 & 0.1576 \\ \cline{3-8} 
                               &                                   & S.D. & 0.0002 & 0.0004     & 0.0062   & 0.0078 & 0.0050 \\ \hline
\end{tabular}
\end{table}


%% Connections to other applications 
% The prediction framework we developed in this paper can also be applied to other ranking problems within an online learning setting. For example, the ranking of items to recommend to customers on Amazon or other e-commerce platforms. In this application, we are ranking different products selling on the platform (whose availability is changing over time, similar to stocks entering/leaving the trading universe in Numerai). Regime shifts can also be found which are characterised by changing consumer preferences over time. We hypothesise dynamic feature projection and model selection methods developed in this paper can improve the robustness of these recommender systems. 
